Slot Games for Detecting Timing Leaks of Programs

In this paper we describe a method for verifying secure information flow of programs, where apart from direct and indirect flows a secret information can be leaked through covert timing channels. That is, no two computations of a program that differ only on high-security inputs can be distinguished by low-security outputs and timing differences. We attack this problem by using slot-game semantics for a quantitative analysis of programs. We show how slot-games model can be used for performing a precise security analysis of programs, that takes into account both extensional and intensional properties of programs. The practicality of this approach for automated verification is also shown.

==> eptcsdata.tex <==
\providecommand{\firstpage}{166}
\providecommand{\publicationstatus}{Gabriele Puppis, Tiziano Villa (Eds.): Fourth International\\ Symposium on Games, Automata, Logics and Formal Verification\\
EPTCS 119, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.119.15}{10.4204/EPTCS.119.15}}

